What do QAOA energies reveal about graphs?

Quantum Approximate Optimization Algorithm (QAOA) is a hybrid classical-quantum algorithm to approximately solve NP optimization problems such as MAX-CUT. We describe a new application area of QAOA circuits: graph structure discovery. We omit the time-consuming parameter-optimization phase and utilize the dependence of QAOA energy on the graph structure for randomly or judiciously chosen parameters to learn about graphs. In the first part, Following up on Wang et. al. and Brandao et. al. we give explicit formulas. We show that the layer-one QAOA energy for the MAX-CUT problem for three regular graphs carries exactly the information: {\em (# of vertices, # of triangles)}. We have calculated our explicit formulas differently from \cite{wang2018quantum}, by developing the notion of the $U$ polynomial of a graph $G$. Many of our discoveries can be interpreted as computing $U(G)$ under various restrictions. The most basic question when comparing the structure of two graphs is if they are isomorphic or not. We find that the QAOA energies separate all non-isomorphic three-regular graphs up to size 18, all strongly regular graphs up to size 26 and the Praust and the smallest Miyazaki examples. We observe that the QAOA energy values can be also used as a proxy to how much graphs differ. Unfortunately, we have also found a sequence of non-isomorphic pairs of graphs, for which the energy gap seems to shrink at an exponential rate as the size grows. Our negative findings however come with a surprise: if the QAOA energies do not measurably separate between two graphs, then both of their energy landscapes must be extremely flat (indistinguishable from constant), already when the number of QAOA layers is intermediately large. This holds due to a remarkable uncoupling phenomenon that we have only deduced from computer simulation.

==> data.tex <==


Ladders G1 = circular, G2 = moebius:

3: [[25.40975322512979], [21.273648093377062], [4.998152292032572], [4.494075398255138]]

[[25.408503063800367], [21.180250017011787], [4.997355879492618], [4.483792758206168]] (15000 repetitions p = 150)

[[25.34247595636], [21.17939648005508], [4.989815230665487], [4.481943211667959]]  (10000 repetitions p = 200)

[[25.477911200360946], [21.530204299764762], [5.002619456235065], [4.520327635257116]]  (5000 repetitions p = 400)

ladder 3, 2000000 trials, level 20
[[25.45780812111802], [5.000840199590206]]

4: [[36.934849773639506], [38.99152601868553], [6.020937251708681], [6.221708867654374]] (1500 repetitions p = 150)

moebius ladder 4, 15000 trials, level 50
[[39.180909541461716], [6.235422667577122]]

moebius ladder 4, 25000 trials, level 50
[[39.133332668891924], [6.231516338948767]]

moebius ladder 4, 250000 trials, level 3
[[38.70961830198712], [6.128979937007156]]

moebius ladder 4, 100000 trials, level 15
[[39.27837615149177], [6.239904946984737]]

moebius ladder 4, 500000 trials, level 10
[[39.420079924793924], [6.2424043618750575]]

5: [[60.07525885230667], [56.3099635568347], [7.741802602565938], [7.493173428262791]] (1500 repetitions p = 150)

6: [[81.07142662653584], [82.81198292475221], [9.000551563635575], [9.097004384436376]] (1500 repetitions p = 150)

7: [[112.01541868474098], [110.23023367045927], [10.582712209825479], [10.49803244048306]] (1500 repetitions p = 150)

G1 = petersen, G2 = ladder 5

[65.54711911219434] [42.29568522578829] [8.070475091762614] [6.501289408011741]  (1500 repetitions p = 150)

G1 = petersen, G2 = circular-ladder 5

[65.72411260540005]  [59.94337462986612]  [8.080900423606828]  [7.73359474077466]  (1500 repetitions p = 150)

[65.0592319553748]  [60.06044871571759]  [8.038558276949958]  [7.741150410843267]   (1500 repetitions p = 150)



Praust1
[[632.5490168821314], [25.150527169070063]]
Praust2
[[625.4754826390357], [25.00950784479846]]
Praust1
[[633.3363222112185], [25.166174167147826]]
Praust2
[[624.8543218466331], [24.997086267135877]]
Praust1
[[638.6518910768905], [25.271562893435984]]
Praust2
[[625.8973432072354], [25.017940426966312]]
single edge
[[0.32780824768311584], [0.49350561893971717]]
single edge
[[0.33979914774706155], [0.5048135132538093]]
single edge
[[0.3247362034252779], [0.49616609362957326]]
single edge
[[0.33892153929084995], [0.5052798148122131]]
[[0.3334987657136235], [0.5002813770552674]]    (1000000 trials)
[[0.3336844772187542], [0.5003527032527376]]    (1000000 trials)

G9 (1000 trials)
[[182.22134641329725], [13.498847989814674]]

nx.circular-ladder-graph(9) (1000 trials)
[[182.93120193048648], [13.525112607608516]]

path 3 (100000 trials)
[[1.1666571527916536], [1.000013169456861]]

path 4 (100000 trials)
[[2.4292582944526813], [1.4985722562280333]]

path 4 (100000 trials)
[[2.429934858987444], [1.4992829003210706]]

star 3 (100000 trials)
[[2.4929000872443976], [1.4973473221195241]]

single edge (level 4, 500000 trials)
[[0.33384893631238655], [0.5009449887902787]]

single edge (level 3, 500000 trials)
[[0.3318257260413289], [0.49983687585108216]]

single edge (level 2, 500000 trials)
[[0.32782591256917937], [0.49984472775865146]]

single edge  (level 1, 500000 trials)
[[0.3119850267912641], [0.499501845254387]]

single edge   (level 0, 500000 trials)
[[0.25], [0.5]]

star 3, 1500000 trials, level 50
[[2.501304196697706], [1.5003402154873784]]

star 4, 150000 trials, level 50
[[4.327850977200241], [1.9989769348117477]]

star 4, 1000000 trials, level 20
[[4.336606827210051], [2.000708867330973]]

3 cycle, 1000000 trials, level 20
[[4.332978232842478], [1.9999713224969349]]

4 cycle, 1000000 trials, level 20
[[4.6644440639608895], [1.9993392380357846]]

star 5, 2000000 trials, level 20
[[6.668689186341289], [2.5001143848817704]]

cycle 5, 2000000 trials, level 20
[[9.668306600023959], [3.000142708009876]]

dragon graph, 2000000 trials, level 20.  (four-cycle + dangling edge)
[[6.384315873775147], [2.499551056777493]]

fiveplus, 2000000 trials, level 20 (five-cycle + (0,2))
[[10.40126896930042], [3.199133278276512]]


Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0,0.05pi]; layers = 100; trials = 5000
[[35.896534371647355], [33.455244645133625], [5.92411996807122], [5.688388083218564], [1.9543921569140394]]
[[61.43035278279339], [59.90607990368924], [7.773636440954111], [7.677318484804273], [1.9750672019124238]]
[[93.0771160708458], [92.08690596314754], [9.605261874418902], [9.553302833331077], [1.6400710744472065]]
[[132.38890496614425], [133.71673723137383], [11.46738017719927], [11.525994445538482], [1.7597217429643024]]
[[180.59767730246745], [180.38157911239693], [13.400895997693954], [13.391617501794453], [2.0599096499731786]]



simple differences:
[0.8818146331369153, 0.9156181548651829, 0.5148736814455296, 0.36650193576275636, 0.27426808536225544]
squared differences:
[1.266481898479173, 1.2548791068160734, 0.43765218342738754, 0.23274790555845315, 0.1271321563340688]

simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.05pi]; layers = 200; trials = 10000 (this is the original algorithm)
[0.8501454002591452, 0.7556767180992567, 0.5616556633967688, 0.3487863444268024, 0.2467711035201326]
squared differences:
[1.1716005112113619, 0.9289271846775359, 0.510370096216404, 0.20019358817703284, 0.10057622791055253]


simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 2pi]; layers = 200; trials = 500 (this is the original algorithm)
[1.0740079130263278, 0.7914107094782457, 0.46817256373054666, 0.2915494045348366, 0.18660303580854942]
squared differences:
[1.8623435952236016, 0.9851452571529513, 0.34416789180386476, 0.1281541638819688, 0.054766759081270024]

simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.15pi]; layers = 200; trials = 2000 (this is the original algorithm)
[1.0546128492165168, 0.8210577013243405, 0.46653310541849, 0.27205488872298167, 0.1817801702548304]
squared differences:
[1.7599499913431769, 1.0531632796445922, 0.34435691497161386, 0.11740624737229673, 0.052374288077519794]

simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.03pi]; layers = 200; trials = 500 (this is the original algorithm)
[0.5963952197023392, 0.6161593897757919, 0.5429882359154445, 0.35119208152018627, 0.27563645018721583]
squared differences:
[0.5678450252637826, 0.6365486020453683, 0.4803201644292572, 0.20155282508435424, 0.12715870297920115]

simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.02pi]; layers = 200; trials = 500 (this is the original algorithm)
simple differences:
[0.4823010004704457, 0.4327998644303858, 0.5015833510901493, 0.3325732902007915, 0.19237539190808728]
squared differences:
[0.3614757265451949, 0.2780680327686142, 0.3931629216000588, 0.18096783256001076, 0.060164763678420864]

simple differences: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.04pi]; layers = 200; trials = 500 (this is the original algorithm)
[0.6942506021104, 0.6990369118697682, 0.5767080906562358, 0.3634729313457762, 0.2706866358655937]
squared differences:
[0.7944090278221271, 0.8050380573586787, 0.5289245776432855, 0.21157462349393003, 0.12128124439745654]



simple differences 25: Ladders and Moebious Ladders 3, ... ,7           the angle sequences were [0, 0.025 etc pi]; layers = 200; trials = 3000 (this is the original algorithm)
[0.5370753092414271, 0.5944475904686105, 0.46596029864916827, 0.2828794377839541, 0.24921420516599246]
squared differences 25:
[0.47357819035637727, 0.5672281878335449, 0.3604878737055883, 0.12946582368288187, 0.10350112386172702]
simple differences 30:
[0.5724561867926601, 0.6055117684200746, 0.5415689320498088, 0.3491557378081729, 0.27407756632965885]
squared differences 30:
[0.532193506130258, 0.6020227469997121, 0.4755480493027885, 0.20506647303137734, 0.12614263697002617]
simple differences 35:
[0.65438786383452, 0.6734406903617164, 0.5484016673163697, 0.36973915670003027, 0.2784795324086542]
squared differences 35:
[0.7044406277729383, 0.7415004884340229, 0.4986857659371174, 0.2228316363675641, 0.12783752901891557]
squared differences 40:
[0.7549249152229439, 0.7162078746023682, 0.5624060898790729, 0.3558828333243816, 0.2739312919182805]
squared differences 40:
[0.9426367939254401, 0.8417013593123158, 0.510639052813199, 0.20896008486965842, 0.1286620346877124]
squared differences 45:
[0.7891899009256207, 0.7355203992842548, 0.5678290687410051, 0.3599911969372405, 0.25829044135936297]
squared differences 45:
[1.012175890901988, 0.8860675370674749, 0.5357599088569343, 0.21189149209892855, 0.1140847006693258]
simple differences 34:
[0.6481682973848191, 0.6432486569699686, 0.5620935244660071, 0.3839325839591934, 0.26691898771817213]
squared differences 34:
[0.6915997099172597, 0.6866457351358695, 0.5141514928948594, 0.2403506028129019, 0.11948391258041954]
simple differences 36:
[0.6672562615327422, 0.6996292705722486, 0.5565059411666113, 0.37601174275858396, 0.275980035232798]
squared differences 36:
[0.7257782328266906, 0.7988266301058071, 0.49937206669184964, 0.22804093503657408, 0.12945697768911735]



level =  291    ...   Ladders and Moebious Ladders 6, the angle sequences is in [0, 2pi]; layers increase from 3, average of 5000 trials
[[0.27995252000565957], [0.12426982935508547]]
level =  231
[[0.2867987624625837], [0.1295152790433795]]
level =  231
[[0.28254093973129446], [0.1261348832355707]]
level =  171
[[0.27916854535237734], [0.12315120564012748]]
level =  171
[[0.28517208466343497], [0.12926709878294243]]


level =  3  ...   Ladders and Moebious Ladders 6, the angle sequences is in [0, 0.035pi]; layers increase from 3, average of 5000 trials
[[1.4039672365129264e-09], [2.96387091049196e-17]]
level =  9
[[2.5068524340683497e-05], [1.9068244507780176e-09]]
level =  15
[[0.00110921694811654], [2.005197223888577e-06]]
level =  21
[[0.004738449387168413], [2.8062669308609776e-05]]
level =  27
[[0.015704779012810154], [0.0005043515714613807]]
level =  33
[[0.05599489693203413], [0.0037649152650451123]]
level =  39
[[0.05475688651556054], [0.004361015475351655]]
level =  45
[[0.10343947557768468], [0.01441317717785029]]
level =  51
[[0.10324019594102758], [0.016407142917869613]]
level =  57
[[0.14425117857001252], [0.032549571757960805]]
level =  63
[[0.16762951404974724], [0.04421254330249563]]
level =  69
[[0.2097844542731979], [0.06490648278710698]]
level =  75
[[0.24128592181320732], [0.0930928848541115]]
level =  81
[[0.27354883021498233], [0.11854939433388603]]
level =  87
[[0.25242426438820215], [0.10032179835086846]]
level =  93
[[0.23654890160720238], [0.08784684918276657]]
level =  99
[[0.22119125322489414], [0.07650111933711175]]
level =  105
[[0.2409418603474107], [0.09377585839916226]]
level =  111
[[0.3036988312609032], [0.15186329979113009]]
level =  117
[[0.33461360160119996], [0.1826820360248022]]
level =  123
[[0.31882408525780964], [0.16302114153714273]]
level =  129
[[0.31069217186452713], [0.15551703333424866]]
level =  135
[[0.30376600529688585], [0.15214234827130263]]
level =  141
[[0.291968829357843], [0.1423588429279071]]
level =  147
[[0.29398759116975737], [0.14207052653933613]]
level =  153
[[0.3093796802592668], [0.15574035083298757]]
level =  159
[[0.31777353034616856], [0.16588473196246964]]
level =  165
[[0.32893435818162686], [0.17483967376905668]]
level =  171
[[0.33955363629672686], [0.19345953118565817]]
level =  177
[[0.35235584475586895], [0.20498519174379626]]
level =  183
[[0.35658921263413906], [0.2121580199324026]]
level =  189
[[0.3771800906759665], [0.2332711053251449]]
level =  195
[[0.3779087925257273], [0.23299211074960244]]
level =  201
[[0.3680727182584941], [0.22250993252231366]]
level =  207
[[0.3606959296261777], [0.21734233979921905]]
level =  213
[[0.3641753421550529], [0.2194820193355702]]
level =  219
[[0.37414179770261796], [0.22972759182526428]]
level =  225
[[0.37851818890689837], [0.2361040856862161]]
level =  231
[[0.3728767788642557], [0.22891204611771718]]
level =  237
[[0.370662476066003], [0.22600846081850787]]
level =  243
[[0.37684751218005047], [0.23853200619280482]]
level =  249
[[0.3796206248633731], [0.24141371519978166]]
level =  255
[[0.3859277528208214], [0.2491689814670433]]
level =  261
[[0.3898702632765216], [0.2487929697103668]]
level =  267
[[0.38760367947667546], [0.25160895707418146]]
level =  273
[[0.3895187359408509], [0.2514124761027606]]
level =  279
[[0.38719757453857523], [0.24859873257935897]]
level =  285
[[0.38972345026128885], [0.24965592286042815]]


...   Ladders and Moebious Ladders 6, the angle sequences is in [0, 0.035pi]; layers increase from 3, average of 5000 trials INDEPENDENT
level =  9
[[2.5235818129949907e-05], [2.0119732802598085e-09]]
level =  15
[[0.0010952526005430939], [1.9211674046681204e-06]]
level =  21
[[0.004692578840891641], [2.7917178895949145e-05]]
level =  27
[[0.015610743787295286], [0.0005049640466020859]]
level =  33
[[0.05635393576012991], [0.003802560748219023]]
level =  39
[[0.05474038961148606], [0.004334911862023859]]
level =  45
[[0.10188873657495799], [0.014038342726732876]]
level =  51
[[0.1030936759174921], [0.01623845407759139]]
level =  57
[[0.14455057862310997], [0.03254883582973028]]
level =  63
[[0.16485787926716208], [0.04277609974339851]]
level =  69
[[0.209306606037678], [0.06484287091133685]]
level =  75
[[0.240746342753299], [0.09153971558723968]]
level =  81
[[0.2728075249121661], [0.11807640921916213]]
level =  87
[[0.2526383754525374], [0.10096317481155281]]
level =  93
[[0.23721715756579892], [0.08782477571368887]]
level =  99
[[0.2191990800670136], [0.07571366534715973]]
level =  105
[[0.23749574683880373], [0.09249421071853829]]
level =  111
[[0.30611264144183437], [0.15595777764322794]]
level =  117
[[0.32894807765361594], [0.17728207507208493]]
level =  123
[[0.31913093428525874], [0.16652171375218755]]
level =  129
[[0.3131755167270533], [0.16001226695469822]]
level =  135
[[0.3084623102672995], [0.1538130512033929]]
level =  141
[[0.2967498889039699], [0.1453329133553103]]
level =  147
[[0.29653183517623716], [0.14453968018218077]]
level =  153
[[0.31186923230262814], [0.15766493576762575]]
level =  159
[[0.3207245391360132], [0.1711880120298751]]
level =  165
[[0.32848350009970884], [0.17881327601845726]]
level =  171
[[0.34315802084844516], [0.1971185970965531]]
level =  177
[[0.3490066221950184], [0.20468633674649944]]
level =  183
[[0.3589859927430607], [0.21281367472155638]]
level =  189
[[0.37683166558444586], [0.23030246045139796]]
level =  195
[[0.3695510588974578], [0.2230709865643637]]
level =  201
[[0.3633672755655244], [0.21760093874273376]]
level =  207
[[0.3682827156300815], [0.22424299540717976]]
level =  213
[[0.37571832529248383], [0.23295617392440673]]
level =  219
[[0.3774246332744363], [0.23792172674240042]]
level =  225
[[0.3784569833148524], [0.23554081804273072]]
level =  231
[[0.3743060115196711], [0.22942753939789817]]
level =  237
[[0.3724187235132504], [0.2292460780791009]]
level =  243
[[0.3793723733342639], [0.23894263590493048]]
level =  249
[[0.3777471939527647], [0.23793635975483568]]
level =  255
[[0.3963288507599685], [0.2587574792402777]]
level =  261
[[0.3928976844764158], [0.25394969824461444]]
level =  267
[[0.3835240591416789], [0.2414051581602213]]
level =  273
[[0.3822129276626774], [0.2389223578770317]]
level =  279
[[0.3902724734232267], [0.24713576639124607]]
level =  285
[[0.39333231801177343], [0.2546376799330067]]   %this can be the last
level =  291
[[0.39460353593137604], [0.25331190660628894]]
level =  297
[[0.3985388786461625], [0.26243101484644155]]
level =  303
[[0.39570419706830096], [0.26236246635476607]]


Ladder Moebius Ladder 6, independent  [lin Ladder, square Moebius, lin, square] 5000 trials [0, 0.035pi];
level =  3 
[[92.03938902918274], [9.589312580052558], [92.03938900392075], [9.589312578806481]]
level =  9
[[139.1595083519448], [11.78515888734181], [139.15890442616308], [11.785134186492046]]
level =  15
[[160.01613132102312], [12.635220429802624], [159.9881406099048], [12.634108708106266]]
level =  21
[[160.70942133082974], [12.645354075565484], [160.6038901826917], [12.64113681339033]]
level =  27
[[162.94489746024271], [12.725227399160634], [163.28958306724067], [12.738729154675735]]
level =  33
[[159.5815639702418], [12.5898260243844], [161.00373847417373], [12.646169642011948]]
level =  39
[[164.5484849704733], [12.780978525427699], [165.0171356052498], [12.799883207587651]]
level =  45
[[179.0545801391549], [13.333041160585024], [176.62634721557387], [13.241873183520552]]
level =  51
[[180.51127691807713], [13.377094944978202], [179.95298635646643], [13.35845698988117]]
level =  57
[[166.02094970470768], [12.807479721284002], [168.59092065640255], [12.911251377347895]]
level =  63
[[149.51421708404698], [12.159614819030516], [148.44002120711565], [12.110474859769317]]
level =  69
[[140.72474993844764], [11.807086499000322], [138.2100563304344], [11.696166289451895]]
level =  75
[[138.394590933033], [11.715156275126569], [141.04389042716343], [11.82905205676987]]
level =  81
[[140.7129451870774], [11.813447894882463], [143.78308406596508], [11.947027569892388]]
level =  87
[[143.54472873858845], [11.93750201018379], [142.8153620855135], [11.906899551043349]]
level =  93
[[141.74523059874923], [11.8619991217957], [140.79403500103464], [11.823028501367784]]
level =  99
[[138.18422521347856], [11.707904304189512], [138.0851776359953], [11.70489206316232]]
level =  105
[[136.84489091353348], [11.65231260372834], [137.6056906289787], [11.6850533293347]]
level =  111
[[141.03890186293896], [11.829880280550654], [144.0693957474833], [11.955442966753218]]
level =  117
[[148.4066609056537], [12.13215555994219], [150.79229382867555], [12.231194726074213]]
level =  123
[[151.52701210048826], [12.260279345031849], [150.0549557618183], [12.20173482957367]]
level =  129
[[146.7230165828336], [12.062446673334415], [144.73978597107], [11.982952068070794]]
level =  135
[[141.41062532483562], [11.844508210413881], [140.94846366098807], [11.828510852415853]]
level =  141
[[138.97046175556156], [11.748444470378637], [139.92703144861443], [11.788777288978862]]
level =  147
[[139.51301421072637], [11.77243382429346], [140.19121572711148], [11.800375186757034]]
level =  153
[[139.2741405418632], [11.76343491264916], [139.59064234898014], [11.776817971401982]]
level =  159
[[138.2704230871456], [11.719372153213364], [138.04113581696623], [11.711152541240827]]
level =  165
[[133.8500271523238], [11.532475240733705], [134.53595706818592], [11.56387017205413]]
level =  171
[[132.2485468247859], [11.465429734694334], [132.1907666527419], [11.463390170844415]]
level =  177
[[132.45276829938953], [11.473312199356528], [132.36589216366346], [11.470074975372698]]
level =  183
[[132.71004805085863], [11.48514012140999], [133.87856000125595], [11.536741679931447]]
level =  189
[[132.6897393807152], [11.485798356715952], [134.3453691608239], [11.557427462339993]]
level =  195
[[133.36168353964504], [11.514821225643947], [134.16555774155378], [11.549862190781948]]
level =  201
[[132.14587007323448], [11.463229424818097], [132.1902486694641], [11.46576930868853]]
level =  207
[[131.16105567983874], [11.420850633218052], [131.53879602625753], [11.43840671034888]]
level =  213
[[130.4225154170906], [11.38856783465553], [131.2063456236241], [11.423809805181316]]
level =  219
[[130.73583404550703], [11.40307396908153], [131.63628087408986], [11.442399921522297]]
level =  225
[[130.3552099173486], [11.387333175533596], [130.81336456713953], [11.407327588166021]]
level =  231
[[129.54549052070612], [11.35205145383708], [129.9570043143424], [11.370445707566741]]
level =  237
[[128.09238844345302], [11.290201888873508], [128.1169395949025], [11.29150181570796]]
level =  243
[[126.704454920065], [11.229762986333697], [126.94592772918469], [11.24093105155237]]
level =  249
[[125.99848802110397], [11.198400599087686], [126.18065421761358], [11.206371689621271]]
level =  255
[[125.91996378183673], [11.195774085817963], [126.14463046441315], [11.205539518119577]]
level =  261
[[125.38183225161156], [11.172953554195804], [125.49109357226241], [11.177539109190402]]
level =  267
[[124.5276077910621], [11.133496142160281], [124.83098051355493], [11.147399052819567]]
level =  273
[[123.87291475955578], [11.105501972090664], [124.18751948905883], [11.119425014038173]]
level =  279
[[123.70405668382344], [11.09819692912401], [124.14946490452036], [11.117892906853038]]
level =  285
[[123.1834443160917], [11.07538120469305], [123.79184799800176], [11.101664944533121]]


Ladder, Moebious 11,   coupled (differences and difference squares) [0, 2pi]; 500
level =  33
[[0.01592588838683465], [0.000421844168055319]]

Ladder, Moebious 6,   coupled (differences and difference squares) [0, 2pi]; 500
level =  33
[[0.2710154302114201], [0.11650529715329597]]

Ladder, Moebious 8,   coupled (differences and difference squares) [0, 2pi]; 500
level =  33
[[0.09753033494870675], [0.014880912047873446]]


cycle 4 repetitions: 5000 ;  level  = 120
[[4.6362085281754295], [1.9955002925537975]]
cycle 5 repetitions: 5000 ;  level  = 120
[[9.77275340753996], [3.016968538097675]]

path 2 repetitions: 400000 ;  level  = 60
[[0.33384442603194014], [0.5002753411047769]]
path 3 repetitions: 400000 ;  level  = 60
[[1.1635434879150646], [0.9985206507539546]]
path4 repetitions: 400000 ;  level  = 60
[[2.4360877621043637], [1.5008563595899005]]
path4 repetitions: 400000 ;  level  = 60
[[2.433218222661823], [1.4998460081612146]]
cycle 5 repetitions: 400000 ;  level  = 60
[[9.675163617919466], [3.001799529933603]]
cycle 5 repetitions: 400000 ;  level  = 60
[[9.660773914711575], [2.9990104261578048]]

path 6 repetitions: 4000 ;  level  = 60
[[6.473625517324527], [2.503529111404483]]
path 7 repetitions: 4000 ;  level  = 60
[[9.196576926377976], [2.9969600359489545]]
path4 repetitions: 4000 ;  level  = 60
[[2.438523959384716], [1.5019717944101796]]
path4 repetitions: 4000 ;  level  = 60
[[2.4322318282458264], [1.4991983621838734]]
cycle 5 repetitions: 4000 ;  level  = 60
[[9.61743202247087], [2.997315197901731]]
cycle 5 repetitions: 4000 ;  level  = 60
[[9.612365260122077], [2.99068119486333]]

cycle 6 repetitions: 500000 ;  level  = 120
[[9.992776041681163], [2.9988595499216406]]
cycle 7 repetitions: 500000 ;  level  = 120
[[17.004054627001985], [4.000385901586501]]

compare coupled circular ladder and moebius ladder
first and second power of the diff; level =  60 rep = 5000 x = 2
param = 6 first = 0.2853204283037331 second = 0.12767921349696132
param = 7 first = 0.18264013708660384 second = 0.052235503452915964
param = 8 first = 0.10253323997088683 second = 0.01667046648608711


first and second power of the diff; level =  60 rep = 5000 x = 2
param = 9 first = 0.06190623967769569 second = 0.005954741678609126

first and second power of the diff; level =  60 rep = 1500 x = 2
param = 10 first = 0.033741406397576494 second = 0.0018078861263049386

first and second power of the diff; level =  60 rep = 15000 x = 2
param = 4 first = 0.8197124293537041 second = 1.069294622531345
param = 5 first = 0.4724082996638822 second = 0.35376603607489315
param = 6 first = 0.2814059803581896 second = 0.12528158426839442


first and second power of the diff; level =  60 rep = 15000 x = 2
param = 3 first = 1.0582902085918984 second = 1.7740771441876937
param = 4 first = 0.8075967359485114 second = 1.0385243012877938




From least distinguishable:

% rep = 200 THE SQUARED DIFFERENCES ARE  1  ...,  12 :
%[1.467281283711082e-30, 9.007213815813513e-29, 5.5787176358176055e-06, 1.5177683234098965e-05, 3.673938943347781e-05, 5.0700018563245815e-05, 8.889022131012836e-05, %0.00014978873295638543, 0.00013172179212796067, 0.0001993715523746198, 0.0002325260945443103, 0.00041890512861222505]
 
%rep = 4000 THE DIFFERENCES ARE  6  ...,  6 :
%[0.00373501]
%rep = 4000 THE SQUARED DIFFERENCES ARE  6  ...,  6 :
%[5.6168437811499424e-05]

% rep = 4000 THE DIFFERENCES ARE  7  ...,  10 :
% [0.0053907  0.00681067 0.00834629 0.00941913]

% rep = 4000 THE SQUARED DIFFERENCES ARE  7  ...,  10 :
% [9.360978136754385e-05, 0.00013041762350669072, 0.00017695469888825939, 0.00019917030427071182]

From structures:


 rep = 500 THE SQUARED DIFFERENCES ARE  3  ...,  10 :
[1.0852901721197886e-06, 6.995562931428708e-06, 2.6575474692098975e-05, 7.451144500691694e-05, 6.431491433599352e-05, 0.0001120180553737008, 0.0008524232737068662, 0.00020125786093507935]

 rep = 500 THE SQUARED DIFFERENCES ARE  3  ...,  10 :
[1.8730586429598294e-06, 8.006876824123963e-06, 2.618171322434443e-05, 4.281398720537843e-05, 7.397754912880712e-05, 0.00012764755656266398, 0.00018990086737769103, 0.00032818518523433817]

 rep = 5000 THE SQUARED DIFFERENCES ARE  3  ...,  3 :
[3.7894016072020043e-06]

 rep = 5000 THE SQUARED DIFFERENCES ARE  3  ...,  3 :
[2.6581957747015427e-06]

 rep = 5000 THE SQUARED DIFFERENCES ARE  3  ...,  3 :
[2.3347634557869734e-06]

rep = 5000 THE SQUARED DIFFERENCES ARE  3  ...,  3 :
[2.4303114117364594e-06]

rep = 5000 THE DIFFERENCES ARE  3  ...,  3 :
[0.00034201]

 rep = 5000 THE DIFFERENCES ARE  3  ...,  3 :
[0.00033047]

 rep = 1000 THE DIFFERENCES ARE  2  ...,  10 :
[7.99893485e-15 3.05662924e-04 1.10267157e-03 2.62028935e-03
 3.58831277e-03 5.41677154e-03 7.02300873e-03 8.07826520e-03
 9.39652786e-03]

 rep = 4000 THE DIFFERENCES ARE  4  ...,  4 :
[0.00123747]

 rep = 4000 THE SQUARED DIFFERENCE
[1.3930692202341641e-05]

 rep = 1000 THE SQUARED DIFFERENCES ARE  2  ...,  10 :
[1.0357112596827708e-28, 1.7384163363976925e-06, 9.107352548278495e-06, 3.644514223064546e-05, 4.51994816999482e-05, 9.781647894327855e-05, 0.00013095792753325472, 0.0001547869056424283, 0.00019931122379074394]

 rep = 4000 THE DIFFERENCES ARE  5  ...,  5 :
[0.00254487]

 rep = 4000 THE SQUARED DIFFERENCES ARE  5  ...,  5 :
[3.2727252251853744e-05]
 
 *************************************************************************************
 
 x = 0.05

 This is individual_separation, rep =  3000

 THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [235.40906860026655]
squared energy for G2: [234.49309272400046]
expected energy for G1: [15.304134341556946]
expected energy for G2: [15.274746993789485]
variance, when independently coupled: [2.3686012717722633]

 The graphs were circular and moebius ladder with parameters lower =  8  upper =  8
 
 
 *************************************************************************************
 
 x = 0.05
 
  This is individual_separation, rep =  2000

 THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [295.3136129944566]
squared energy for G2: [295.4950085689508]
expected energy for G1: [17.146734028384188]
expected energy for G2: [17.152359036131323]
variance, when independently coupled: [2.5947448596155027]

 The graphs were circular and moebius ladder with parameters lower =  9  upper =  9
 
 **************************************************************************************
 
 x = 0.05
 
  THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [181.63953580938872]
squared energy for G2: [179.76381701847035]
expected energy for G1: [13.43776476758077]
expected energy for G2: [13.369594868762361]
variance, when independently coupled: [2.0884110592920706]

 The graphs were circular and moebius ladder with parameters lower =  7  upper =  7
 
 
 **********************************************************************************
 
 x = 0.05
 
  This is individual_separation, rep =  5000

 THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [132.42232068092264]
squared energy for G2: [133.1990223113408]
expected energy for G1: [11.468222800131516]
expected energy for G2: [11.504087399773471]
variance, when independently coupled: [1.7584681666878055]

 The graphs were circular and moebius ladder with parameters lower =  6  upper =  6
 
*********************************************************************
 
x = 0.05
  
This is individual_separation, rep =  5000

 THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [36.00656118596506]
squared energy for G2: [33.49682113342375]
expected energy for G1: [5.934132778094307]
expected energy for G2: [5.689910483378546]
variance, when independently coupled: [1.9740137117106968]

 The graphs were circular and moebius ladder with parameters lower =  3  upper =  3
 
 ********************************************************************
 x = 2
 
  This is individual_separation, rep =  5000

 THE DIFFERENCES ARE  100  ...,  100 :
squared energy for G1: [25.614371777887406]
squared energy for G2: [21.428645593926284]
expected energy for G1: [5.015879541228581]
expected energy for G2: [4.513336174663188]
variance, when independently coupled: [1.766316209453791]

 The graphs were circular and moebius ladder with parameters lower =  3  upper =  3
 
 *********************************************************************
 
 
 This is individual_separation, rep =  5000 layers = 100

 THE DIFFERENCES ARE  50  ...,  50 :
squared energy for G1: [1.159641604115403]
squared energy for G2: [1.1663167826827947]
expected energy for G1: [0.9973950343630895]
expected energy for G2: [1.0003546392175116]
variance, when independently coupled: [0.330460887282946]

 The graphs were nx.path(3), nx.path(3)
 
 ***********************************************************************
 
 
  This is individual_separation, rep =  100000

 THE DIFFERENCES ARE  1  ...,  4 (layers):
squared energy for G1: [1.0760923784181242, 1.11708051977135, 1.1430153860880043, 1.1562690963498117]
squared energy for G2: [1.0778096906825567, 1.1222351547257734, 1.141514343912211, 1.1504671962968198]
expected energy for G1: [0.9987939203943176, 0.9989062183938344, 1.0017886584563296, 1.003033939340225]
expected energy for G2: [0.9996924625556342, 1.0011645862453737, 1.0014988956655833, 1.0000459599540776]
variance, when independently coupled: [0.15692856137149835, 0.239176612824735, 0.2779492597315749, 0.30057621517860067]

 The graphs were nx.path_graph(3), nx.path_graph(3)
[1.0760923784181242, 1.11708051977135, 1.1430153860880043, 1.1562690963498117]
[1.0778096906825567, 1.1222351547257734, 1.141514343912211, 1.1504671962968198]
[0.9987939203943176, 0.9989062183938344, 1.0017886584563296, 1.003033939340225]
[0.9996924625556342, 1.0011645862453737, 1.0014988956655833, 1.0000459599540776]
[0.15692856137149835, 0.239176612824735, 0.2779492597315749, 0.30057621517860067]

***************************************************

 This is individual_separation, rep =  100000

 THE DIFFERENCES ARE  1  ...,  4 :
squared energy for G1: [2.371878963908337, 2.417366729204885, 2.429870364072898, 2.4311972872978176]
squared energy for G2: [2.375125873329904, 2.4190082676244424, 2.4334448322087363, 2.438055161052296]
expected energy for G1: [1.4989639738512075, 1.5012300318748426, 1.4998155408142197, 1.4979785014311255]
expected energy for G2: [1.5001749692951742, 1.501652004195262, 1.5014605514858839, 1.5001979021423089]
variance, when independently coupled: [0.24958837034462622, 0.32772482458337926, 0.35948745820559935, 0.37472403774760554]

 The graphs were nx.path_graph(3), nx.path_graph(3)
[2.371878963908337, 2.417366729204885, 2.429870364072898, 2.4311972872978176]
[2.375125873329904, 2.4190082676244424, 2.4334448322087363, 2.438055161052296]
[1.4989639738512075, 1.5012300318748426, 1.4998155408142197, 1.4979785014311255]
[1.5001749692951742, 1.501652004195262, 1.5014605514858839, 1.5001979021423089]
[0.24958837034462622, 0.32772482458337926, 0.35948745820559935, 0.37472403774760554]

***********************************************************

 This is individual_separation, rep =  1000

 THE DIFFERENCES ARE  1  ...,  4 :
squared energy for G1: [4.1820879311148635, 4.280417637926902, 4.505473183079045, 4.678310173145515]
squared energy for G2: [4.236406146207108, 4.456128148434112, 4.75378226931959, 4.792692962536689]
expected energy for G1: [1.9880293790520387, 1.9526881904738214, 1.9759237017759126, 2.0147312931491292]
expected energy for G2: [1.9981627093786, 1.984888857153315, 2.0497246137941056, 2.036338829659939]
variance, when independently coupled: [0.4736817365802164, 0.9848077248282969, 1.1590565593801294, 1.265652008541096]

 The graphs were nx.path_graph(3), nx.path_graph(3)
[4.1820879311148635, 4.280417637926902, 4.505473183079045, 4.678310173145515]
[4.236406146207108, 4.456128148434112, 4.75378226931959, 4.792692962536689]
[1.9880293790520387, 1.9526881904738214, 1.9759237017759126, 2.0147312931491292]
[1.9981627093786, 1.984888857153315, 2.0497246137941056, 2.036338829659939]
[0.4736817365802164, 0.9848077248282969, 1.1590565593801294, 1.265652008541096]

**************************************************************
 
 
 This is individual_separation, rep =  100000

 THE DIFFERENCES ARE  1  ...,  4 :
squared energy for G1: [4.677363748040373, 4.82263083661121, 4.861091273702856, 4.862167817778718]
squared energy for G2: [4.677591262362909, 4.820442211368071, 4.858959013731999, 4.863048860092841]
expected energy for G1: [2.124763275380828, 2.1555236934027326, 2.1655894049994773, 2.1665518422563803]
expected energy for G2: [2.12495866327572, 2.154853785650264, 2.1648718140919825, 2.166954383552919]
variance, when independently coupled: [0.32488675154211144, 0.3533962664038466, 0.34360335987566515, 0.33557865432732825]

 The graphs were dragon, dragon
[4.677363748040373, 4.82263083661121, 4.861091273702856, 4.862167817778718]
[4.677591262362909, 4.820442211368071, 4.858959013731999, 4.863048860092841]
[2.124763275380828, 2.1555236934027326, 2.1655894049994773, 2.1665518422563803]
[2.12495866327572, 2.154853785650264, 2.1648718140919825, 2.166954383552919]
[0.32488675154211144, 0.3533962664038466, 0.34360335987566515, 0.33557865432732825]
 
 **************************************************************
the energy is: (2.5+0j)
the energy is: (2.5+0j)
the energy is: (2.5+0j)
the energy is: (2.34375+0j)
the energy is: (2.2265625+0j)
the energy is: (2.1484375+0j)
the energy is: (2.09716796875+0j)
the energy is: (2.0635986328125+0j)
the energy is: (2.0416259765625+0j)
the energy is: (2.0272445678710938+0j)
the energy is: (2.017831802368164+1.4224732503009818e-16j)

***************************************************


 This is individual_separation, rep =  10000

 THE DIFFERENCES ARE  1  ...,  5 :
squared energy for G1: [22.68565277429407, 23.804761304097894, 24.553349290834877, 24.942866031377886, 25.095074153956773]
squared energy for G2: [22.619507318684644, 23.567871666180498, 24.47129174874469, 24.907572127645775, 25.131659429984495]
expected energy for G1: [4.691827297959262, 4.798102707021618, 4.877869492125813, 4.92306572497081, 4.944920352280894]
expected energy for G2: [4.68547486722945, 4.776217514973709, 4.870749889961937, 4.921585553176335, 4.94902059466968]
variance, when independently coupled: [1.3382823210403458, 1.5390685944395486, 1.5068764555385812, 1.3918598603158188, 1.2817082590624835]

 The graphs were circ. ladder 3, circ. ladder 3
[22.68565277429407, 23.804761304097894, 24.553349290834877, 24.942866031377886, 25.095074153956773]
[22.619507318684644, 23.567871666180498, 24.47129174874469, 24.907572127645775, 25.131659429984495]
[4.691827297959262, 4.798102707021618, 4.877869492125813, 4.92306572497081, 4.944920352280894]
[4.68547486722945, 4.776217514973709, 4.870749889961937, 4.921585553176335, 4.94902059466968]
[1.3382823210403458, 1.5390685944395486, 1.5068764555385812, 1.3918598603158188, 1.2817082590624835]

*************************************************

(4.5+0j)
(4.3125+0j)
(4.2041015625+0j)
(4.1292572021484375+0j)
(4.080656290054321+0j)
(4.050103034824133+0j)
(4.031138496065978+0j)
(4.019405640537116+0j)
(4.012139220685538+0j)
(4.007625745985566+0j)

***************************************************

(2.5+0j)
(2.5+0j)
(2.65625+0j)
(2.7734375+0j)
(2.8515625+0j)
(2.90283203125+0j)
(2.9364013671875+0j)
(2.9583740234375+0j)
(2.972755432128906+0j)
(2.982168197631839+3.7730235602495554e-17j)

**************************************************

level = 1
(2.5+0j)
level = 2
(2.65625+0j)
level = 3
(2.7734375+0j)
level = 4
(2.8515625+0j)
level = 5
(2.90283203125+0j)
level = 6
(2.9364013671875+0j)
level = 7
(2.9583740234375+0j)
level = 8
(2.972755432128906+0j)
level = 9
(2.9821681976318377+0j)
level = 10
(2.988328933715826+0j)

ladder 4:

level = 1
(6+0j)
level = 2
(6+0j)

star 4:

level = 1
(6+0j)
level = 2
(6+0j)
US-153968-MP:Shou-Yu mario.szegedy$ !!
python3 -m examples.GRAPH_ISOMORPHISM.sigma
level = 1
(2+0j)
level = 2
(2+0j)
level = 3
(2+0j)
level = 4
(2+0j)
level = 5
(2+0j)
level = 6
(2+0j)
level = 7
(2+0j)
level = 8
(2+0j)
level = 9
(2.0000000000000013+0j)
level = 10
(2.0000000000000013+0j)
level = 11
(2.0000000000000027+0j)
level = 12
(2.0000000000000013+0j)
level = 13
(2.000000000000001+0j)
level = 14
(1.9999999999999996+0j)
level = 15
(2.0000000000000018+0j)
level = 16
(1.9999999999999993+0j)
level = 17
(1.9999999999999982+0j)
level = 18
(1.9999999999999987+0j)
level = 19
(1.9999999999999998+0j)
level = 20
(2+0j)


star 5:


level = 1
(2.5+0j)
level = 2
(2.5+0j)
level = 3
(2.5+0j)
level = 4
(2.5+0j)
level = 5
(2.5+0j)
level = 6
(2.5+0j)
level = 7
(2.5+0j)
level = 8
(2.4999999999999996+0j)
level = 9
(2.5000000000000018+0j)
level = 10
(2.500000000000004+0j)
level = 11
(2.500000000000003+0j)
level = 12
(2.500000000000001+0j)
level = 13
(2.5000000000000053+0j)
level = 14
(2.4999999999999973+0j)
level = 15
(2.499999999999992+0j)
level = 16
(2.4999999999999827+0j)
level = 17
(2.4999999999999925+0j)
level = 18
(2.4999999999999876+0j)
level = 19
(2.4999999999999827+0j)
level = 20
(2.4999999999999876+0j)

 This is individual_separation, rep =  10000

 THE DIFFERENCES ARE  1  ...,  5 :
squared energy for G1: [6.65773035018752, 7.6110432944865085, 8.31457084604548, 8.778456313781652, 9.051841483925916]
squared energy for G2: [6.620843717231682, 7.609979576348157, 8.279763965822946, 8.763212143326756, 9.151175498831359]
expected energy for G1: [2.5028139792415214, 2.6570724635369354, 2.7737043954263805, 2.8521215636807997, 2.897561835179042]
expected energy for G2: [2.4957912216795672, 2.656266297524522, 2.7681104465102595, 2.8465640820035167, 2.912572256402577]
variance, when independently coupled: [0.7855717496434096, 1.1052388008874345, 1.2384945868460537, 1.3041748557454653, 1.3243005580504494]

 The graphs were 5 cycle, 5 cycle
[6.65773035018752, 7.6110432944865085, 8.31457084604548, 8.778456313781652, 9.051841483925916]
[6.620843717231682, 7.609979576348157, 8.279763965822946, 8.763212143326756, 9.151175498831359]
[2.5028139792415214, 2.6570724635369354, 2.7737043954263805, 2.8521215636807997, 2.897561835179042]
[2.4957912216795672, 2.656266297524522, 2.7681104465102595, 2.8465640820035167, 2.912572256402577]
[0.7855717496434096, 1.1052388008874345, 1.2384945868460537, 1.3041748557454653, 1.3243005580504494]


 THE DIFFERENCES ARE  6  ...,  10 :
squared energy for G1: [9.28688514528473, 9.379469937946785, 9.507154734946077, 9.57688731018579, 9.489522440775914]
squared energy for G2: [9.306805948597574, 9.376840122124879, 9.46290371470709, 9.523479962458214, 9.548720854550245]
expected energy for G1: [2.9373172494771884, 2.951952882906146, 2.9758492292113776, 2.983905394255217, 2.969486542195643]
expected energy for G2: [2.9400188196602763, 2.9511533260699805, 2.9653339528879656, 2.9769713299929608, 2.979656786345321]
variance, when independently coupled: [1.3221551083309215, 1.3329789224909838, 1.3212849335412074, 1.334365652425756, 1.3421418404974617]

 The graphs were 5 cycle, 5 cycle
[9.28688514528473, 9.379469937946785, 9.507154734946077, 9.57688731018579, 9.489522440775914]
[9.306805948597574, 9.376840122124879, 9.46290371470709, 9.523479962458214, 9.548720854550245]
[2.9373172494771884, 2.951952882906146, 2.9758492292113776, 2.983905394255217, 2.969486542195643]
[2.9400188196602763, 2.9511533260699805, 2.9653339528879656, 2.9769713299929608, 2.979656786345321]
[1.3221551083309215, 1.3329789224909838, 1.3212849335412074, 1.334365652425756, 1.3421418404974617]

***************************************************
 
In Alibaba I have joined an optimistic, ambitious, and hard-working team, which has brought out
the best of my talents. I have never felt more creative and innovative. My ideas are cherished and embraced.
In our circle of knowledgeable colleagues I have learned important aspects of quantum computing
that were in my blind spot. Joining AQL was a choice that has tremendously fostered my scientific growth.

 
 
 **************
 
 
 
 
 *************
 
 circular ladder 3
 
 
 level = 1
(4.6875+0j)


(0.024169921875+0j)(0.024169921875+0j)(0.024169921875+0j)

(0.024169921875+0j)(0.024169921875+0j)(0.024169921875+0j)

(0.024169921875+0j)(0.024169921875+0j)(0.024169921875+0j)




(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)(0.012451171875+0j)

level = 2
(4.7958984375+0j)


(0.024951934814453125+0j)(0.024951934814453125+0j)(0.024951934814453125+0j)

(0.024951934814453125+0j)(0.024951934814453125+0j)(0.024951934814453125+0j)

(0.024951934814453125+0j)(0.024951934814453125+0j)(0.024951934814453125+0j)




(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)(0.011402130126953125+0j)

level = 3
(4.8707427978515625+0j)


(0.024093806743621826+0j)(0.024093806743621826+0j)(0.024093806743621826+0j)

(0.024093806743621826+0j)(0.024093806743621826+0j)(0.024093806743621826+0j)

(0.024093806743621826+0j)(0.024093806743621826+0j)(0.024093806743621826+0j)




(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)(0.011068522930145264+0j)

level = 4
(4.919343709945679+0j)


(0.02317110914736986+0j)(0.02317110914736986+0j)(0.02317110914736986+0j)

(0.02317110914736986+0j)(0.02317110914736986+0j)(0.02317110914736986+0j)

(0.02317110914736986+0j)(0.02317110914736986+0j)(0.02317110914736986+0j)




(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)(0.010899615474045277+0j)

level = 5
(4.949896965175867+0j)


(0.0224639219668461+0j)(0.0224639219668461+0j)(0.0224639219668461+0j)

(0.0224639219668461+0j)(0.0224639219668461+0j)(0.0224639219668461+0j)

(0.0224639219668461+0j)(0.0224639219668461+0j)(0.0224639219668461+0j)




(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)(0.010780071883345954+0j)

level = 6
(4.968861503934022+0j)


(0.02196465171005002+0j)(0.02196465171005002+0j)(0.02196465171005002+0j)

(0.02196465171005002+0j)(0.02196465171005002+0j)(0.02196465171005002+0j)

(0.02196465171005002+0j)(0.02196465171005002+0j)(0.02196465171005002+0j)




(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)(0.010687725657817282+0j)

level = 7
(4.980594359462884+0j)


(0.02162009395193465+0j)(0.02162009395193465+0j)(0.02162009395193465+0j)

(0.02162009395193465+0j)(0.02162009395193465+0j)(0.02162009395193465+0j)

(0.02162009395193465+0j)(0.02162009395193465+0j)(0.02162009395193465+0j)




(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)(0.010616678804705515+0j)

level = 8
(4.9878607793144605+0j)


(0.021383100301966718+0j)(0.021383100301966718+0j)(0.021383100301966718+0j)

(0.021383100301966718+0j)(0.021383100301966718+0j)(0.021383100301966718+0j)

(0.021383100301966718+0j)(0.021383100301966718+0j)(0.021383100301966718+0j)




(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)(0.01056307012169172+0j)

level = 9
(4.992374254014434+0j)


(0.021219527861816863+0j)(0.021219527861816863+0j)(0.021219527861816863+0j)

(0.021219527861816828+0j)(0.021219527861816828+0j)(0.021219527861816828+0j)

(0.02121952786181678+0j)(0.02121952786181678+0j)(0.021219527861816787+0j)




(0.010523281560601753+0j)(0.010523281560601753+0j)(0.010523281560601755+0j)(0.010523281560601753+0j)(0.010523281560601751+0j)(0.010523281560601753+0j)

(0.01052328156060176+0j)(0.01052328156060176+0j)(0.01052328156060176+0j)(0.01052328156060176+0j)(0.010523281560601757+0j)(0.010523281560601757+0j)

(0.010523281560601736+0j)(0.010523281560601732+0j)(0.010523281560601736+0j)(0.010523281560601734+0j)(0.010523281560601734+0j)(0.010523281560601734+0j)

(0.010523281560601741+0j)(0.010523281560601743+0j)(0.010523281560601741+0j)(0.010523281560601741+0j)(0.01052328156060174+0j)(0.01052328156060174+0j)

(0.010523281560601722+0j)(0.010523281560601724+0j)(0.010523281560601722+0j)(0.01052328156060172+0j)(0.01052328156060172+0j)(0.010523281560601718+0j)

(0.010523281560601718+0j)(0.010523281560601717+0j)(0.010523281560601717+0j)(0.010523281560601717+0j)(0.010523281560601715+0j)(0.010523281560601713+0j)

level = 10
(4.99518816847215+0j)


(0.021105995366021146+0j)(0.021105995366021146+0j)(0.021105995366021153+0j)

(0.0211059953660211+0j)(0.0211059953660211+0j)(0.021105995366021098+0j)

(0.021105995366021136+0j)(0.021105995366021136+0j)(0.02110599536602114+0j)




(0.010494080798622072+0j)(0.010494080798622072+0j)(0.010494080798622072+0j)(0.010494080798622069+0j)(0.010494080798622072+0j)(0.010494080798622072+0j)

(0.010494080798622072+0j)(0.010494080798622076+0j)(0.010494080798622069+0j)(0.010494080798622076+0j)(0.010494080798622069+0j)(0.010494080798622069+0j)

(0.010494080798622072+0j)(0.010494080798622069+0j)(0.010494080798622072+0j)(0.010494080798622076+0j)(0.010494080798622069+0j)(0.010494080798622069+0j)

(0.010494080798622041+0j)(0.010494080798622045+0j)(0.010494080798622041+0j)(0.010494080798622045+0j)(0.010494080798622041+0j)(0.010494080798622041+0j)

(0.01049408079862203+0j)(0.010494080798622034+0j)(0.01049408079862203+0j)(0.010494080798622038+0j)(0.010494080798622027+0j)(0.010494080798622024+0j)

(0.010494080798622065+0j)(0.010494080798622065+0j)(0.010494080798622062+0j)(0.010494080798622065+0j)(0.010494080798622055+0j)(0.010494080798622055+0j)

level = 11
(4.996949555560471+0j)


(0.02102672149320944+0j)(0.02102672149320944+0j)(0.021026721493209454+0j)

(0.02102672149320946+0j)(0.02102672149320946+0j)(0.021026721493209458+0j)

(0.021026721493209527+0j)(0.021026721493209527+0j)(0.021026721493209527+0j)




(0.010472799057404234+0j)(0.010472799057404236+0j)(0.010472799057404234+0j)(0.010472799057404236+0j)(0.01047279905740423+0j)(0.010472799057404227+0j)

(0.010472799057404229+0j)(0.010472799057404234+0j)(0.010472799057404225+0j)(0.01047279905740423+0j)(0.010472799057404222+0j)(0.010472799057404222+0j)

(0.010472799057404227+0j)(0.01047279905740423+0j)(0.010472799057404223+0j)(0.010472799057404232+0j)(0.01047279905740422+0j)(0.010472799057404222+0j)

(0.010472799057404206+0j)(0.010472799057404208+0j)(0.010472799057404203+0j)(0.010472799057404204+0j)(0.0104727990574042+0j)(0.010472799057404206+0j)

(0.010472799057404173+0j)(0.01047279905740417+0j)(0.010472799057404171+0j)(0.010472799057404175+0j)(0.010472799057404164+0j)(0.010472799057404166+0j)

(0.010472799057404208+0j)(0.0104727990574042+0j)(0.010472799057404206+0j)(0.010472799057404203+0j)(0.010472799057404203+0j)(0.010472799057404203+0j)

level = 12
(4.998056714878623+0j)


(0.020971052748478682+0j)(0.020971052748478686+0j)(0.02097105274847868+0j)

(0.020971052748478686+0j)(0.020971052748478693+0j)(0.02097105274847868+0j)

(0.020971052748478717+0j)(0.020971052748478713+0j)(0.02097105274847871+0j)




(0.01045734995761329+0j)(0.010457349957613287+0j)(0.010457349957613287+0j)(0.010457349957613285+0j)(0.010457349957613282+0j)(0.010457349957613283+0j)

(0.01045734995761327+0j)(0.010457349957613282+0j)(0.010457349957613275+0j)(0.010457349957613271+0j)(0.01045734995761327+0j)(0.01045734995761327+0j)

(0.010457349957613273+0j)(0.010457349957613275+0j)(0.010457349957613273+0j)(0.010457349957613278+0j)(0.010457349957613262+0j)(0.010457349957613266+0j)

(0.01045734995761327+0j)(0.01045734995761327+0j)(0.010457349957613262+0j)(0.010457349957613271+0j)(0.010457349957613268+0j)(0.010457349957613275+0j)

(0.010457349957613268+0j)(0.010457349957613268+0j)(0.01045734995761327+0j)(0.010457349957613275+0j)(0.010457349957613278+0j)(0.010457349957613278+0j)

(0.01045734995761328+0j)(0.010457349957613278+0j)(0.010457349957613276+0j)(0.010457349957613282+0j)(0.01045734995761328+0j)(0.010457349957613287+0j)

level = 13
(4.9987556497203185+0j)


(0.02093175767749172+0j)(0.02093175767749171+0j)(0.020931757677491707+0j)

(0.02093175767749174+0j)(0.020931757677491742+0j)(0.020931757677491735+0j)

(0.02093175767749177+0j)(0.020931757677491745+0j)(0.02093175767749176+0j)




(0.010446157079067452+0j)(0.010446157079067448+0j)(0.010446157079067441+0j)(0.010446157079067438+0j)(0.010446157079067446+0j)(0.010446157079067443+0j)

(0.010446157079067434+0j)(0.01044615707906743+0j)(0.01044615707906743+0j)(0.010446157079067427+0j)(0.010446157079067417+0j)(0.01044615707906742+0j)

(0.010446157079067432+0j)(0.010446157079067443+0j)(0.010446157079067436+0j)(0.01044615707906745+0j)(0.010446157079067429+0j)(0.010446157079067432+0j)

(0.01044615707906743+0j)(0.010446157079067424+0j)(0.010446157079067422+0j)(0.010446157079067429+0j)(0.010446157079067432+0j)(0.010446157079067432+0j)

(0.010446157079067412+0j)(0.01044615707906741+0j)(0.010446157079067406+0j)(0.010446157079067412+0j)(0.010446157079067413+0j)(0.010446157079067417+0j)

(0.010446157079067412+0j)(0.010446157079067422+0j)(0.010446157079067419+0j)(0.010446157079067419+0j)(0.010446157079067427+0j)(0.01044615707906743+0j)

level = 14
(4.99919886092928+0j)


(0.020903892409340163+0j)(0.02090389240934015+0j)(0.020903892409340135+0j)

(0.02090389240934016+0j)(0.020903892409340166+0j)(0.02090389240934014+0j)

(0.020903892409340125+0j)(0.02090389240934009+0j)(0.02090389240934011+0j)




(0.01043805370103243+0j)(0.010438053701032426+0j)(0.010438053701032428+0j)(0.010438053701032422+0j)(0.010438053701032431+0j)(0.010438053701032428+0j)

(0.010438053701032408+0j)(0.01043805370103241+0j)(0.01043805370103241+0j)(0.010438053701032405+0j)(0.010438053701032393+0j)(0.010438053701032403+0j)

(0.01043805370103241+0j)(0.01043805370103241+0j)(0.01043805370103241+0j)(0.010438053701032415+0j)(0.010438053701032403+0j)(0.0104380537010324+0j)

(0.010438053701032395+0j)(0.010438053701032398+0j)(0.010438053701032395+0j)(0.010438053701032398+0j)(0.0104380537010324+0j)(0.010438053701032401+0j)

(0.010438053701032374+0j)(0.010438053701032384+0j)(0.010438053701032375+0j)(0.010438053701032388+0j)(0.010438053701032393+0j)(0.0104380537010324+0j)

(0.010438053701032375+0j)(0.010438053701032386+0j)(0.010438053701032379+0j)(0.010438053701032384+0j)(0.010438053701032393+0j)(0.010438053701032393+0j)

level = 15
(4.999481239256841+0j)


(0.020884052075405963+0j)(0.02088405207540596+0j)(0.02088405207540595+0j)

(0.020884052075405987+0j)(0.02088405207540599+0j)(0.020884052075405963+0j)

(0.020884052075406046+0j)(0.020884052075406025+0j)(0.02088405207540605+0j)




(0.01043218684618331+0j)(0.010432186846183304+0j)(0.010432186846183304+0j)(0.010432186846183304+0j)(0.010432186846183297+0j)(0.0104321868461833+0j)

(0.010432186846183307+0j)(0.010432186846183305+0j)(0.01043218684618331+0j)(0.010432186846183295+0j)(0.010432186846183274+0j)(0.010432186846183284+0j)

(0.01043218684618331+0j)(0.010432186846183314+0j)(0.010432186846183317+0j)(0.010432186846183317+0j)(0.010432186846183307+0j)(0.0104321868461833+0j)

(0.0104321868461833+0j)(0.010432186846183307+0j)(0.0104321868461833+0j)(0.010432186846183321+0j)(0.010432186846183312+0j)(0.010432186846183314+0j)

(0.010432186846183269+0j)(0.01043218684618328+0j)(0.010432186846183265+0j)(0.010432186846183286+0j)(0.010432186846183288+0j)(0.010432186846183286+0j)

(0.010432186846183286+0j)(0.010432186846183283+0j)(0.010432186846183286+0j)(0.010432186846183284+0j)(0.010432186846183291+0j)(0.010432186846183288+0j)US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ 
US-153968-MP:Shou-Yu mario.szegedy$ !!
python3 -m examples.GRAPH_ISOMORPHISM.sigma


moebius ladder 3:


level = 1
(4.5+0j)
empty list





(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)(0.010986328125+0j)

level = 2
(4.5+0j)
empty list





(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)(0.009693145751953125+0j)

level = 3
(4.5+0j)
empty list





(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)(0.009367763996124268+0j)

level = 4
(4.5+0j)
empty list





(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)(0.009286385960876942+0j)

level = 5
(4.5+0j)
empty list





(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)(0.009266040942748077+0j)

level = 6
(4.5+0j)
empty list





(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)(0.009260954680257782+0j)

level = 7
(4.5+0j)
empty list





(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)(0.009259683114510864+0j)

level = 8
(4.499999999999998+0j)
empty list





(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)(0.009259365223072191+0j)

level = 9
(4.499999999999998+0j)
empty list





(0.009259285750212488+0j)(0.009259285750212487+0j)(0.00925928575021249+0j)(0.009259285750212488+0j)(0.009259285750212488+0j)(0.00925928575021249+0j)(0.009259285750212487+0j)(0.00925928575021249+0j)(0.009259285750212487+0j)

(0.009259285750212481+0j)(0.009259285750212483+0j)(0.009259285750212488+0j)(0.009259285750212483+0j)(0.009259285750212487+0j)(0.009259285750212487+0j)(0.00925928575021249+0j)(0.00925928575021249+0j)(0.009259285750212488+0j)

(0.009259285750212487+0j)(0.009259285750212487+0j)(0.009259285750212483+0j)(0.009259285750212485+0j)(0.009259285750212487+0j)(0.009259285750212485+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)

(0.00925928575021248+0j)(0.009259285750212483+0j)(0.009259285750212485+0j)(0.009259285750212481+0j)(0.009259285750212485+0j)(0.009259285750212481+0j)(0.009259285750212483+0j)(0.009259285750212488+0j)(0.009259285750212481+0j)

(0.009259285750212485+0j)(0.009259285750212481+0j)(0.009259285750212487+0j)(0.009259285750212485+0j)(0.009259285750212488+0j)(0.009259285750212488+0j)(0.009259285750212488+0j)(0.009259285750212492+0j)(0.00925928575021249+0j)

(0.009259285750212481+0j)(0.009259285750212483+0j)(0.009259285750212487+0j)(0.009259285750212481+0j)(0.009259285750212485+0j)(0.009259285750212483+0j)(0.009259285750212487+0j)(0.009259285750212488+0j)(0.009259285750212483+0j)

(0.009259285750212485+0j)(0.009259285750212485+0j)(0.009259285750212485+0j)(0.009259285750212483+0j)(0.009259285750212487+0j)(0.009259285750212485+0j)(0.009259285750212485+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)

(0.00925928575021247+0j)(0.009259285750212471+0j)(0.009259285750212473+0j)(0.009259285750212475+0j)(0.009259285750212471+0j)(0.009259285750212473+0j)(0.009259285750212473+0j)(0.009259285750212475+0j)(0.009259285750212475+0j)

(0.009259285750212485+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)(0.009259285750212483+0j)(0.009259285750212481+0j)(0.009259285750212481+0j)(0.00925928575021248+0j)(0.00925928575021248+0j)

level = 10
(4.499999999999992+0j)
empty list





(0.009259265881997575+0j)(0.009259265881997578+0j)(0.009259265881997577+0j)(0.00925926588199758+0j)(0.009259265881997575+0j)(0.00925926588199758+0j)(0.009259265881997577+0j)(0.009259265881997573+0j)(0.009259265881997573+0j)

(0.009259265881997575+0j)(0.009259265881997582+0j)(0.009259265881997577+0j)(0.009259265881997573+0j)(0.009259265881997578+0j)(0.009259265881997577+0j)(0.009259265881997577+0j)(0.00925926588199757+0j)(0.009259265881997577+0j)

(0.009259265881997582+0j)(0.009259265881997589+0j)(0.009259265881997587+0j)(0.009259265881997584+0j)(0.009259265881997582+0j)(0.009259265881997584+0j)(0.009259265881997587+0j)(0.009259265881997584+0j)(0.009259265881997584+0j)

 
 
 ****************************************
 
 Ladder 2:
 
 
level = 1
(2+0j)
.....
(4+0j)
{(0.09765625+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.04296875+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.03125+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06640625+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.09765625+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 2
(2+0j)
.....
(4+0j)
{(0.11352539+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03588867+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.015625+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06469727+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.11352539+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 3
(2+0j)
.....
(4+0j)
{(0.12025452+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03312683+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.0078125+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06349182+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12025452+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 4
(2+0j)
.....
(4+0j)
{(0.12304783+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.0320158+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00390625+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06292057+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12304783+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 5
(2+0j)
.....
(4+0j)
{(0.1241985+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03156346+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00195312+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06267458+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.1241985+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 6
(2+0j)
.....
(4+0j)
{(0.12467116+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03137846+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00097656+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06257192+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12467116+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 7
(2+0j)
.....
(4+0j)
{(0.12486512+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03130267+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00048828+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06252954+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12486512+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 8
(2+0j)
.....
(4+0j)
{(0.12494468+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.0312716+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00024414+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06251212+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12494468+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 9
(2+0j)
.....
(4+0j)
{(0.12497731+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03125886+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (0.00012207+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06250497+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.12497731+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


level = 10
(2+0j)
.....
(4+0j)
{(0.1249907+0j): ((0, 0, 0, 0), (0, 0, 0, 0))}
(2+0j)
{(0.03125363+0j): ((0, 1, 1, 1), (0, 1, 1, 1)), (6.104e-05+0j): ((0, 1, 1, 1), (0, 1, 0, 1)), (0.06250204+0j): ((0, 1, 0, 1), (0, 1, 0, 1))}
0j
{(0.1249907+0j): ((0, 1, 1, 0), (0, 1, 1, 0))}


***************************************************************

ladder 4

level = 1
(6+0j)
.....
(12+0j)
{(0.0188961+0j): ((0, 0, 0, 0, 0, 0, 0, 0), (0, 0, 0, 0, 0, 0, 0, 0))}
(9+0j)
{(0.00406837+0j): ((0, 1, 1, 1, 1, 1, 1, 1), (0, 1, 1, 1, 1, 1, 1, 1))}
(8+0j)
{(0.00403404+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00429344+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00803185+0j): ((0, 1, 1, 0, 0, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0))}
(6+0j)
{(0.003088+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 1, 0)), (0.00261497+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 0, 1)), (0.00214195+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00562096+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 1, 0, 1)), (0.0028286+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (-0.00017738+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00351524+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0))}
(7+0j)
{(0.00266457+0j): ((0, 1, 1, 1, 0, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 0))}
(5+0j)
{(0.00266457+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 1, 1, 0, 0))}
(3+0j)
{(0.00406837+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 1, 0, 1, 0))}
(4+0j)
{(0.00403404+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00429344+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 0, 1, 0, 0, 1)), (0.00803185+0j): ((0, 1, 1, 0, 1, 0, 0, 1), (0, 1, 1, 0, 1, 0, 0, 1))}
0j
{(0.0188961+0j): ((0, 1, 0, 1, 1, 0, 1, 0), (0, 1, 0, 1, 1, 0, 1, 0))}


level = 2
(6+0j)
.....
(12+0j)
{(0.02721451+0j): ((0, 0, 0, 0, 0, 0, 0, 0), (0, 0, 0, 0, 0, 0, 0, 0))}
(9+0j)
{(0.00433485+0j): ((0, 1, 1, 1, 1, 1, 1, 1), (0, 1, 1, 1, 1, 1, 1, 1))}
(8+0j)
{(0.00363793+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00334911+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00953273+0j): ((0, 1, 1, 0, 0, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0))}
(6+0j)
{(0.00285644+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 1, 0)), (0.00204012+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 0, 1)), (0.0012238+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00608643+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 1, 0, 1)), (0.00231509+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (-0.00173122+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00340638+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0))}
(7+0j)
{(0.00224711+0j): ((0, 1, 1, 1, 0, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 0))}
(5+0j)
{(0.00224711+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 1, 1, 0, 0))}
(3+0j)
{(0.00433485+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 1, 0, 1, 0))}
(4+0j)
{(0.00363793+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00334911+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 0, 1, 0, 0, 1)), (0.00953273+0j): ((0, 1, 1, 0, 1, 0, 0, 1), (0, 1, 1, 0, 1, 0, 0, 1))}
0j
{(0.02721451+0j): ((0, 1, 0, 1, 1, 0, 1, 0), (0, 1, 0, 1, 1, 0, 1, 0))}

#############################################################

Moebius ladder 4

level = 1
(6+0j)
.....
(12+0j)
{(0.0168314+0j): ((0, 0, 0, 0, 0, 0, 0, 0), (0, 0, 0, 0, 0, 0, 0, 0))}
(9+0j)
{(0.00394344+0j): ((0, 1, 1, 1, 1, 1, 1, 1), (0, 1, 1, 1, 1, 1, 1, 1))}
(8+0j)
{(0.00534153+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 1, 0)), (0.00362492+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00382328+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00373936+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00384617+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00743198+0j): ((0, 1, 1, 0, 0, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0))}
(6+0j)
{(0.00312901+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 1, 0, 1)), (0.00278568+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 0, 1, 1)), (0.00090122+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00187016+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00152683+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00354099+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 1, 0, 1, 1)), (0.00071049+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00167942+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00243473+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00276279+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00180912+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00161839+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 0, 0, 1, 0)), (0.0026865+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00249577+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00340366+0j): ((0, 1, 1, 1, 0, 0, 1, 0), (0, 1, 1, 1, 0, 0, 1, 0))}
(7+0j)
{(0.00391293+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 1, 1, 0, 0)), (0.00185299+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 0, 1, 1, 0)), (0.00272274+0j): ((0, 1, 1, 1, 0, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 0))}
(5+0j)
{(0.00308895+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 1, 0, 1, 0)), (0.00159359+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 0, 1, 0, 1)), (0.00302792+0j): ((0, 1, 1, 1, 0, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 1))}
(3+0j)
{(0.00519466+0j): ((0, 1, 1, 0, 1, 1, 0, 1), (0, 1, 1, 0, 1, 1, 0, 1))}
(4+0j)
{(0.00430393+0j): ((0, 1, 1, 0, 1, 0, 1, 0), (0, 1, 1, 0, 1, 0, 1, 0)), (0.00336552+0j): ((0, 1, 1, 0, 1, 0, 1, 0), (0, 1, 0, 1, 0, 1, 0, 1)), (0.00865269+0j): ((0, 1, 0, 1, 0, 1, 0, 1), (0, 1, 0, 1, 0, 1, 0, 1))}
(2+0j)
{(0.00819492+0j): ((0, 1, 1, 0, 1, 0, 0, 1), (0, 1, 1, 0, 1, 0, 0, 1))}

 
 
level = 2
(6.0665283203125+0j)
.....
(12+0j)
{(0.02565616+0j): ((0, 0, 0, 0, 0, 0, 0, 0), (0, 0, 0, 0, 0, 0, 0, 0))}
(9+0j)
{(0.00401936+0j): ((0, 1, 1, 1, 1, 1, 1, 1), (0, 1, 1, 1, 1, 1, 1, 1))}
(8+0j)
{(0.00479769+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 1, 1, 1, 0)), (0.00264363+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00254706+0j): ((0, 1, 1, 1, 1, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00417645+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 1, 0, 1, 1, 1)), (0.00338368+0j): ((0, 1, 1, 1, 0, 1, 1, 1), (0, 1, 1, 0, 0, 1, 1, 0)), (0.00910845+0j): ((0, 1, 1, 0, 0, 1, 1, 0), (0, 1, 1, 0, 0, 1, 1, 0))}
(6+0j)
{(0.00283937+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 1, 0, 1)), (0.00215124+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 0, 1, 1)), (0.00037087+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00125898+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00057085+0j): ((0, 1, 1, 1, 1, 1, 0, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.0032688+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 1, 0, 1, 1)), (9.41e-06+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00063549+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00175306+0j): ((0, 1, 1, 1, 1, 0, 1, 1), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00406851+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 1, 0, 0, 0)), (0.00137534+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00101388+0j): ((0, 1, 1, 1, 1, 0, 0, 0), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00257504+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 1, 0, 0)), (0.00195156+0j): ((0, 1, 1, 1, 0, 1, 0, 0), (0, 1, 1, 1, 0, 0, 1, 0)), (0.00313377+0j): ((0, 1, 1, 1, 0, 0, 1, 0), (0, 1, 1, 1, 0, 0, 1, 0))}
(7+0j)
{(0.00398157+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 1, 1, 0, 0)), (0.00114206+0j): ((0, 1, 1, 1, 1, 1, 0, 0), (0, 1, 1, 1, 0, 1, 1, 0)), (0.00222038+0j): ((0, 1, 1, 1, 0, 1, 1, 0), (0, 1, 1, 1, 0, 1, 1, 0))}
(5+0j)
{(0.00263484+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 1, 0, 1, 0)), (0.0008615+0j): ((0, 1, 1, 1, 1, 0, 1, 0), (0, 1, 1, 1, 0, 1, 0, 1)), (0.0029459+0j): ((0, 1, 1, 1, 0, 1, 0, 1), (0, 1, 1, 1, 0, 1, 0, 1))}
(3+0j)
{(0.00516932+0j): ((0, 1, 1, 0, 1, 1, 0, 1), (0, 1, 1, 0, 1, 1, 0, 1))}
(4+0j)
{(0.00420937+0j): ((0, 1, 1, 0, 1, 0, 1, 0), (0, 1, 1, 0, 1, 0, 1, 0)), (0.0019478+0j): ((0, 1, 1, 0, 1, 0, 1, 0), (0, 1, 0, 1, 0, 1, 0, 1)), (0.01289137+0j): ((0, 1, 0, 1, 0, 1, 0, 1), (0, 1, 0, 1, 0, 1, 0, 1))}
(2+0j)
{(0.00926271+0j): ((0, 1, 1, 0, 1, 0, 0, 1), (0, 1, 1, 0, 1, 0, 0, 1))}
 
 *******************
 
 ladder vs moebius 4
 
 
This was correlated separation
THE DIFFERENCES ARE  layers: 1  ...,  4 :
[5.77604631e-16 1.82829465e-01 3.28906493e-01 4.22381022e-01]



This was independent separation
THE DIFFERENCES ARE  1  ...,  4 :
[1.19351192 1.28134593 1.23630357 1.16983933]

********************

second order single edge

les.GRAPH_ISOMORPHISM.sigma2
level = 1
(0.3125+0j)
level = 2
(0.328125+0j)
level = 3
(0.33203125+0j)
level = 4
(0.3330078125+0j)
level = 5
(0.333251953125+0j)
level = 6
(0.33331298828125+0j)
level = 7
(0.3333282470703125+0j)
level = 8
(0.3333320617675781+0j)
level = 9
(0.33333301544189453+0j)
level = 10
(0.33333325386047363+0j)

level = 1
(0.3125+0j)
level = 2
(0.328125+0j)
level = 3
(0.33203125+0j)
level = 4
(0.3330078125+0j)
level = 5
(0.333251953125+0j)

level = 1
(0.3125+0j)
level = 2
(0.328125+0j)
level = 3
(0.33203125+0j)
level = 4
(0.3330078125+0j)
level = 5
(0.333251953125+0j)


*********************

second order path of length 2

level = 1
(1.078125+0j)
level = 2
(1.119384765625+0j)
level = 3
(1.1393013000488281+0j)
level = 4
(1.1500959992408752+0j)
level = 5
(1.1563878180459142+0j)





\subsection{Another proof of the Triangle Theorem}


We will show:

\begin{lemma}\label{mainlemma} $E_{0} + E_{2} = 2 E_{1}$.
\end{lemma}
Together with Equations (\ref{EQA}),  (\ref{EQB}) and $m = N_{0} + N_{1} + N_{2}$ this yields:

\begin{equation}
E = N_{0}E_{0} + N_{1}{E_{0}+E_{2}\over 2} + N_{2}E_{2} \; =\;  m E_{0} + {3\over 2} (E_{2} - E_{0}) t
\end{equation}

\begin{corollary}
For fixed angles the one-level QAOA for 3-regular graph is a linear function of the size of the graph and its number of the triangles.
\end{corollary}

\begin{proof}[Proof of Lemma \ref{mainlemma}:] The energy term associated with a Type 0 edge is represented by 
a tensor network $T_{0}$ (Figure \ref{}). The value computed by this tensor network is the $U$ polynomial 
of the graph in Figure \ref{} with the replacements indicated on the figure. The very same tensor network 
with a little modification can be used to compute $T_{1}$ and $T_{2}$.

\begin{figure}[H]
\centering
\includegraphics[width=0.5\textwidth]{zero3}
\caption{$U(G)$ of the graph $G$ in the figure with replacements indicated on the edges
is zero if and only if $2T_{1} = T_{0} + T_{2}$. This annulling rule will be central in proving Theorem \ref{anulemma}.\label{zero0}}
\end{figure}


